Learning Task Automata for Reinforcement Learning using Hidden Markov Models

Training reinforcement learning (RL) agents using scalar reward signals is often infeasible when an environment has sparse and non-Markovian rewards. Moreover, handcrafting these reward functions before training is prone to misspecification, especially when the environment's dynamics are only partially known. This paper proposes a novel pipeline for learning non-Markovian task specifications as succinct finite-state `task automata' from episodes of agent experience within unknown environments. We leverage two key algorithmic insights. First, we learn a product MDP, a model composed of the specification's automaton and the environment's MDP (both initially unknown), by treating the product MDP as a partially observable MDP and using the well-known Baum-Welch algorithm for learning hidden Markov models. Second, we propose a novel method for distilling the task automaton (assumed to be a deterministic finite automaton) from the learnt product MDP. Our learnt task automaton enables the decomposition of a task into its constituent sub-tasks, which improves the rate at which an RL agent can later synthesise an optimal policy. It also provides an interpretable encoding of high-level environmental and task features, so a human can readily verify that the agent has learnt coherent tasks with no misspecifications. In addition, we take steps towards ensuring that the learnt automaton is environment-agnostic, making it well-suited for use in transfer learning. Finally, we provide experimental results compared with two baselines to illustrate our algorithm's performance in different environments and tasks.

==> Figures/results/experiment_1.tex <==
\begin{tikzpicture}
    \begin{axis}[
        ymode=log,
        ylabel style={at={(axis description cs:0.08,.5)},anchor=south},
        xlabel=Number of DFA states,
        ylabel=Time to convergence (s),
        xmin=0, xmax=40,
        ymin=1, ymax=60000,
        ytick pos=left,
        xtick pos=bottom,
        xtick={10,20,30},
        xticklabels={3,4,5},
        legend style={at={(0.8,0.1)},anchor=south,legend cell align=left}
        ]
    \addplot[smooth,mark=*,blue] plot coordinates {
        (10,39)
        (20,363)
        (30,1635)
    };
    \addlegendentry{3x3}
    
    \addplot[smooth,color=d_red,mark=x]
        plot coordinates {
            (10,619)
            (20,3388)
            (30,16914)
        };
    \addlegendentry{4x4}
    
    \addplot[smooth,color=d_green,mark=square]
        plot coordinates {
            (10,2351)
            (20,15896)
            (30,41270)
        };
    \addlegendentry{5x5}
    \end{axis}
\end{tikzpicture}

==> Figures/results/experiment_2.tex <==
\begin{tikzpicture}
    \begin{axis}[
        ymode=log,
        ylabel style={at={(axis description cs:0.08,.5)},anchor=south},
        xlabel=Grid Dimensions,
        ylabel=Time to convergence (s),
        xmin=0, xmax=40,
        ymin=1, ymax=10000,
        ytick pos=left,
        xtick pos=bottom,
        xtick={10,20,30},
        xticklabels={3x3,4x4,5x5},
        legend style={at={(0.8,0.1)},anchor=south,legend cell align=left}
        ]
    \addplot[smooth,mark=*,blue] plot coordinates {
        (10,106)
        (20,1840)
        (30,6279)
    };
    \addlegendentry{Uniform}
    
    \addplot[smooth,color=d_red,mark=x]
        plot coordinates {
            (10,39)
            (20,619)
            (30,2351)
        };
        
    \addplot[smooth,color=d_green,mark=square]
        plot coordinates {
            (10,39)
            (20,626)
            (30,2259)
        };    
    \addlegendentry{Spatial}
    \end{axis}
\end{tikzpicture}

==> Figures/results/experiment_3_bar.tex <==
\begin{tikzpicture}
 
\begin{axis} [ybar = .05cm,
    bar width = 12pt,
    ymode=log,
    ylabel style={at={(axis description cs:0.08,.5)},anchor=south},
    xlabel=Number of TA states,
    ylabel=Time to convergence (s),
    xmin=0, xmax=40,
    ymin=1, ymax=100000,
    ytick pos=left,
    xtick pos=bottom,
    xtick={10,20,30},
    xticklabels={3,4,5},
    legend style={at={(0.18,0.75)},anchor=south,legend cell align=left}
]

\addplot[color=blue,fill=blue,opacity=0.6] coordinates {(10,26) (20,382) (30,5233)};
\addlegendentry{Ours}
\addplot[color=d_red,fill=d_red,opacity=0.6] coordinates {(10,661) (20,3825) (30,38025)};
\addlegendentry{BF}
\addplot[color=d_green,fill=d_green,opacity=0.6] coordinates {(10,2625) (20,16820) (30,68978)};
\addlegendentry{5x5}
\end{axis}
 
\end{tikzpicture}
